Efficient Planning in a Compact Latent Action Space

Planning-based reinforcement learning has shown strong performance in tasks in discrete and low-dimensional continuous action spaces. However, planning usually brings significant computational overhead for decision-making, and scaling such methods to high-dimensional action spaces remains challenging. To advance efficient planning for high-dimensional continuous control, we propose Trajectory Autoencoding Planner (TAP), which learns low-dimensional latent action codes with a state-conditional VQ-VAE. The decoder of the VQ-VAE thus serves as a novel dynamics model that takes latent actions and current state as input and reconstructs long-horizon trajectories. During inference time, given a starting state, TAP searches over discrete latent actions to find trajectories that have both high probability under the training distribution and high predicted cumulative reward. Empirical evaluation in the offline RL setting demonstrates low decision latency which is indifferent to the growing raw action dimensionality. For Adroit robotic hand manipulation tasks with high-dimensional continuous action space, TAP surpasses existing model-based methods by a large margin and also beats strong model-free actor-critic baselines.

==> tex/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
    \item The method itself, 
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}
\end{enumerate}

==> tex/introduction_arxiv.tex <==
\section{Introduction}
Large generative models have achievement remarkable success for language and image data~\citep{DevlinCLT19,BrownMRSKDNSSAA20,HoJA20,abs-2204-06125} since the self-supervised learning set absorbs the rich information in the whole dataset.
The learned generative models are also very flexible and can be used in varied downstream tasks by sampling from conditional distributions or finetuning.
%In reinforcement learning, recent methods~\citep{janner2021offline,janner2022diffuser} applied these generative models in natural language processing and computer vision.
Recently, such generative models in natural language processing and computer vision are also introduced to Reinforcement Learning (RL)~\citep{janner2021offline,janner2022diffuser}.
These generative sequence modelling methods directly treat the trajectory as a sequence which involves states, actions, rewards and returns without hard-coded causal graph-structured following the Markov Decision Process.
With powerful generative models like Transformer and Diffusion model, Trajectory Transformer~\citep{janner2021offline} and Diffuser~\citep{janner2022diffuser} can accurately plan into more than a hundred future steps in an offline continuous control setting, whereas conventional one-step shooting models quickly collapses~\citep{janner2021offline} due to the compounding error.
Since also modelling the actions that generate the data, generative sequence modelling methods can easily alleviate the out-of-distribution (OOD) actions problem in the offline RL setting.
The accurate sequence modelling ability leads to strong performance in offline model-based continuous control on D4RL~\citep{abs-2004-07219}.


However, prior works like Trajectory Transformer~\citep{janner2021offline} and Diffuser~\citep{janner2022diffuser} have high decision latency which prevents real-time decision making.
This is because sampling and planning with these models involved more unroll steps compared to the traditional shooting models.
In order to model the distribution, rather than the expectation of the trajectories, TT builds a discrete representation of the trajectories so that the distribution of the trajectories is categorical.
TT discretizes each dimension separately for continuous control tasks and treats each dimension as an individual token, yielding $O(D^3)$ sampling cost for the state and action dimension $D$.
On the other hand, the notoriously slow sampling speed for the Diffusion model because of a large number of denoising steps is also extended by the Diffuser.
%And what's more, the planning of Diffuser happens in a latent space whose size is proportional to $D$, which means the computational cost also grows with state-action dimensionality with $O(D)$ complexity. 

To unlock real-time high-dimensional continuous control with a trajectory generative model, we consider constructing a compact latent action space for planning, where the size of this action space will not grow with $D$.
%Since the marginal distribution of the trajectories is not needed for planning, representing the whole distribution with discrete random variables is not necessary.
In this paper we propose the Trajectory Autoencoding Planner (TAP), which learned the mapping between the \emph{the possible future trajectories} given the current state and sequence of discrete latent codes, using a state-conditioned Vector Quantised Variational AutoEncoder (VQ-VAE).
As illustrated in \cref{fig:prior_modelling}, the distribution of these latent codes is then modelled autoregressively with a Transformer, again conditioned on the current state.
During inference, instead of sampling the next state/action/reward sequentially, TAP samples latent codes, reconstructs the trajectory via the decoder, and executes the first action in the trajectory with the highest objective score.
Every single latent code of TAP corresponds to a branch of the tree of possible trajectories, continuing and forking from the existing trajectory.
The forking is caused by different actions sampled from the behaviour policy and the uncertainty of the model.
The number of latent variables to model the forking of the trajectories can be much smaller than that of representing the whole trajectories.
For example, for a deterministic environment with a deterministic policy, an ideal TAP model should not need extra latent codes to reconstruct the trajectory given a starting state.
In practice, TAP uses a single discrete latent variable to model multiple ($L=3$) steps of transitions, creating a compact latent space for downstream planning.
The computational cost of TAP planning is thus $O(C)$ regarding dimensionality $D$ when $D$ is not much larger than the embedding size.

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.43\textwidth}
        \includegraphics[width=\textwidth]{img/prior_modelling.png}
        \caption{{TAP Modelling}}
        \label{fig:prior_modelling}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{img/scaledim.png}
        \caption{{Decision Latency}}
        \label{fig:scaledim}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{img/performdim.png}
        \caption{{Relative Performance}}
        \label{fig:perfomdim}
    \end{subfigure}
    \caption{(a) gives an overview of TAP modelling, where blocks represent the latent codes. (b) shows decision time growth with the dimensionality $D$. Tests are done on a single GPU. The number of planning steps for (b) is 15 and both models apply a beam search with a beam width of 64 and expansion factor of 4. (c) shows the relative performance between TAP and other baselines when dealing with tasks with increasing action dimensionalities.}
    \label{fig:computation}
\end{figure}

We evaluate TAP extensively in the offline RL setting.
Our results on low-dimensional locomotion control tasks show that TAP enjoys competitive performance as strong model-based, model-free actor-critic, and sequence modelling baselines.
On tasks with higher dimensionality, TAP not only surpasses model-based methods like TT but also significantly outperforms strong actor-critic baselines.
In \cref{fig:perfomdim}, we show how the relative performance between TAP and baselines changes according to the dimensionality of the action space. 
We can see TAP perform increasingly better when the dimension of actions grows, and it surpass both model-based and model-free methods in higher action dimension control tasks.
This can be explained by the innate difficulty of policy optimization in a high-dimensional action space, which is avoided by TAP since its planning happens in a low-dimensional discrete latent space.
At the same time, the sampling and planning of TAP are significantly faster than the Transformer-based generative model:
the decision time of TAP meets the requirement of deployment on a real robot (20Hz)~\citep{gato}, while TT is much slower and the latency grows along the state-action dimensionality in \cref{fig:scaledim}.

To sum up, TAP is a planning-based sequence modelling method.
Similar to previous sequence modelling methods like TT, the latent structure of the model is not limited to the MDP causal graph, which leads to lower compounding error when predicting multiple steps in future.
The main contribution of this work is:
1) We propose to use a state-conditioned VQ-VAE to model the trajectories, which constructs a compact latent action space for downstream planning. 
2) We propose to leverage the probability estimation of the generative model to explicitly prevent the agent from choosing actions that either deviate too much from the behaviour policy or lead to low confidence plans.
3) Empirical evaluation in offline RL setting shows TAP efficiently scales up to higher state-action dimensionality, and surpasses previous model-based and model-free methods in high-dimensional continuous control.


==> tex/methodyuandong.tex <==
\iffalse
\subsection{Issues with Rollout Decomposition}

\def\vs{\pmb{s}}
\def\va{\pmb{a}}
\def\vz{\pmb{z}}
\def\vx{\pmb{x}}

Consider the following trajectory $\tau$ of length $T$, sampled from an MDP consists of a sequence of states, actions, rewards and return-to-go $R_t = \sum_{i=t}\gamma^{i-t} r_i$ as proxies for future rewards:
\begin{equation}
    \tau = \left(\pmb{s}_1, \pmb{a}_1, r_1, R_1, \pmb{s}_2, \pmb{a_2}, r_2, R_2,  \ldots, \pmb{s}_T, \pmb{a}_T, r_T, R_T \right)
\end{equation}
A popular way used in many model-based reinforcement learning (RL) approaches~\cite{} to model $\tau$ is to use the following \emph{rollout decomposition}:
\begin{equation}
    p(\tau|\pmb{s} = \pmb{s_1}) = \prod_{t=1}^{T-1} \mu(\pmb{a}_t | \pmb{s}_t) p(\pmb{s}_{t+1} | \pmb{s}_{t}, \pmb{a}_{t}) p(r_t|\pmb{s}_t) 
\end{equation}
where $\mu$ is the behaviour policy and $p$ is the dynamics of the environment. We pointed out that this rollout decomposition, while popular, has some major shortcomings: the model does not directly capture the relationship within raw action sequences $(\va_1, \va_2, \ldots, \va_{T-1})$. Instead, it is implicitly modelled by the behaviour policy, another unknown quality to be estimated from offline data. Furthermore, the correlation among action $\va_t$, reward $r_t$ and reward-to-go $R_t$ is also not modeled in the decomposition and requires separate models to capture (e.g., value/policy function).
\fi

\subsection{Latent Action Model for Planning}
In this work, we propose \emph{latent-action} modelling that captures such correlation directly without a known behaviour model, to achieve faster and more reliable long-horizon planning.
The idea is simple: we represent an input trajectory $\tau$ as an initial state $\vs_1$ plus a sequence of \emph{conditional latent action codes} $z = (\vz_1, \ldots, \vz_M)$
, where $M \ll T$, i.e., the length $M$ of latent code sequence can be much smaller than the trajectory length $T$, due to substantial correlations among actions (in particular consecutive actions).
Therefore, planning in the latent space yields much shorter horizon and thus faster planning. We emphasize that conditional modeling is important since the latent structure can be very different given different initial state $\vs_1$.

To connect the latent representation $(\vs_1, z)$ with the observable trajectory $\tau$, we train a pair of encoder $g$ and decoder $h$. The encoder $g$ takes the trajectory $\tau$ as the input and outputs the latent representation, while the decoder takes the latent representation and reconstructs $\tau$. 

The planning stage using TAP is straightforward. Given the initial state $\vs_1$, we use a sampler $p(z|\vs_1)$ to generate the conditional latent code $z$, then call the decoder $h$ to generate a trajectory $\tau$, which contains its estimated reward and return-to-go:
\begin{equation}
z \sim p(\cdot|\vs_1),\quad\quad \tau \sim h(\cdot|\vs_1,z) \label{eq:sampling}
\end{equation}
Then trajectories with high rewards and high probability are picked (Sec.~\ref{}). The sampler $p(z|\vs_1)$ is learned from the offline trajectories, once their latent codes was computed by the encoder. 
The overall pipeline of TAP is illustrated in \cref{fig:traintest}.

Our latent-action modelling also mitigates another problem in rollout decomposition, in which the final state $\vs_T$ needs to be computed $T-1$ times, based on previous estimation results. This leads to compound errors that scale with the horizon length $T$. In comparison, our latent-action model first estimates a latent sequence, then decodes the entire trajectory with the sequence in one shot. These extra decoding steps make the reconstruction much smoother, which is also adopted in previous transformer-based models (e.g., Trajectory Transformer).
